A Principled Solution to the Disjunction Problem of Diagrammatic Query Representations

Finding unambiguous diagrammatic representations for first-order logical formulas and relational queries with arbitrarily nested disjunctions has been a surprisingly long-standing unsolved problem. We refer to this problem as the disjunction problem (of diagrammatic query representations). This work solves the disjunction problem. Our solution unifies, generalizes, and overcomes the shortcomings of prior approaches for disjunctions. It extends the recently proposed Relational Diagrams and is identical for disjunction-free queries. However, it can preserve the relational patterns and the safety for all well-formed Tuple Relational Calculus (TRC) queries, even with arbitrary disjunctions. Additionally, its size is proportional to the original TRC query and can thus be exponentially more succinct than Relational Diagrams.

==> datalabmacros.tex <==

\usepackage{anyfontsize}	%
\usepackage[T1]{fontenc} %
\usepackage{amsmath}
\usepackage{graphicx} %
\usepackage{url}
\usepackage{enumitem} %
\newcommand{\bmmax}{3}	%
\usepackage{bm} %
\usepackage{upgreek} %
\usepackage{soul} %
\usepackage{bbding} %
\usepackage{pifont} %

\usepackage{listings} %

\usepackage{tabularx} %
\usepackage{booktabs} %
\usepackage{multirow}
\usepackage{hhline} %
\usepackage{diagbox}

\usepackage{booktabs}  %

\usepackage{tikz} %
\usetikzlibrary{positioning}

\usepackage{wasysym}	%



\RequirePackage{etoolbox}	%
\newcommand{\iflabelexists}[3]{\ifcsundef{r@#1}{#3}{#2}}


\usepackage{wrapfig}
\usepackage{cutwin}



\usepackage{adjustbox}
\def\eox{\unskip\kern 10pt{\unitlength1pt\linethickness{.4pt}$\diamondsuit${}}} %

\usepackage{easybmat} %


\usepackage{rotating}		%






\usepackage{svg}


\usepackage{pgfplotstable} %


\sloppy %





\let\subcaption\relax
\let\subfloat\relax
\usepackage{subcaption}		%
\captionsetup[figure]{font=small}		%
\captionsetup[table]{font+=small}		%
\captionsetup[subfigure]{font+=small}	%
\captionsetup[figure]{aboveskip=3pt}
\captionsetup[subfigure]{aboveskip=5pt}







\usepackage[ruled,noend,linesnumbered]{algorithm2e} %

\DontPrintSemicolon     %
\SetNlSty{}{}{}                %
\SetAlgoInsideSkip{smallskip}   %
\SetAlCapSkip{1.5mm}             %
\setlength{\algomargin}{1.5mm}    %
\SetInd{1.5mm}{1.5mm}             %

\SetAlFnt{\small}			%
\SetAlCapFnt{\small}		%
\SetAlCapNameFnt{\small}









\newcommand{\todo}[1]{{\color{red}[\textbf{TODO}:{#1}]}} %
\newcommand{\wolf}[1]{{{\color{red}{[\textbf{wg}: #1]}}}} %
\newcommand{\deprecate}[1]{{{\color{gray}{#1}}}} %
\newcommand{\out}[1]{{\color{gray}\textbf{OUT}: #1}}


\newcommand{\later}[1]{{\color{blue}\textbf{LATER}: #1}}

\newcommand{\laterr}[1]{}

\newcommand{\revision}[1]{{\color{blue}{#1}}}



\newcommand{\hide}[1]{{}} 		%




\newcommand{\addformat}[1]{\textcolor{blue}{#1}} 
\newcommand{\removeformat}[1]{\textcolor{red}{#1}}



\newcommand{\mkclean}{
    \renewcommand{\out}[1]{\hide}
    \renewcommand{\todo}{\hide}
    \renewcommand{\deprecate}{\hide}
    \renewcommand{\later}{\hide{}}
    \renewcommand{\wolf}[1]{\hide{}}
    \renewcommand{\cody}[1]{\hide}	
    \renewcommand{\cd}[2]{\hide}	
}
















\usepackage[capitalise,nameinlink]{cleveref} %

\crefname{algocf}{Alg.}{Algs.}
\Crefname{algocf}{Algorithm}{Algorithms}
\crefalias{AlgoLine}{line}%
\crefname{property}{Property}{Properties}

\crefformat{equation}{(#2#1#3)}						%
\crefrangeformat{equation}{(#3#1#4) to~(#5#2#6)}
\crefmultiformat{equation}{(#2#1#3)}%
{ and~(#2#1#3)}{, (#2#1#3)}{ and~(#2#1#3)}



\AtEndPreamble{%
    \hypersetup{colorlinks,
      linkcolor=purple,
      citecolor=blue,
      urlcolor=ACMDarkBlue,
      filecolor=ACMDarkBlue,
      pdfcreator = {},
      }}










	
	\usepackage[normalem]{ulem} %
	\newcommand\highl{\bgroup\markoverwith
	  {\textcolor{yellow}{\rule[-.5ex]{2pt}{2.5ex}}}\ULon}





\usepackage{marginnote}
\newcommand{\rebuttal}[2]{\marginnote{\textbf{\textcolor{blue}{#1}}}{\color{blue}#2}}
\newcommand{\new}[1]{{\color{blue}{#1}}}








\usepackage{tcolorbox}		%
\tcbuselibrary{breakable,skins}		%


\tcbset{examplestyle/.style={
		enhanced jigsaw,	%
		colback=blue!05,	%
		colframe=blue!10,	%
		arc=2mm,			%
		boxrule=1pt,		%
		left=1mm,
		right=1mm,
		left skip=0mm,  %
		right skip=0mm, %
		top=1mm,		%
		bottom=1mm,		%
		breakable,		%
		parbox = false,		%
		before={\par\pagebreak[0]\vspace{1mm}\parindent=0pt},
		after={\par\pagebreak[0]\vspace{1mm}\parindent=0pt},				
		bottomrule = 0mm,
		boxsep = 0mm,					%
		topsep at break=0pt,			%
		bottomsep at break=0pt,			%
		pad at break=0mm,
		pad before break=0mm,		
		pad after break=1mm,		
		bottomrule at break=0mm,
		toprule at break=0mm,		
		}}

\tcolorboxenvironment{example}{examplestyle}



\newtheoremstyle{abcd}%
  {}%
  {}%
  {\upshape}%
  {}%
  {\itshape}%
  {.}%
  {.5em}%
  {}%

\theoremstyle{abcd}
\newtheorem{example}{Example}




\tcbset{theoremstyle/.style={
		enhanced jigsaw,	%
		colback=white,	%
		colframe=black,	%
		arc=2mm,			%
		boxrule=1pt,		%
		left=1mm,
		right=1mm,
		left skip=0mm,  %
		right skip=0mm, %
		top=1mm,		%
		bottom=1mm,		%
		breakable,		%
		parbox = false,		%
		before={\par\pagebreak[0]\vspace{1mm}\parindent=0pt},
		after={\par\pagebreak[0]\vspace{1mm}\parindent=0pt},				
		boxsep = 0mm,					%
		topsep at break=0pt,			%
		bottomsep at break=0pt,			%
		pad at break=0mm,
		pad before break=0mm,		
		pad after break=1mm,		
		bottomrule at break=0mm,
		toprule at break=0mm,		
		}}




\newtheoremstyle{abcd}%
  {}%
  {}%
  {\itshape}%
  {}%
  {\scshape}%
  {.}%
  {.5em}	%
  {\thmname{#1}\thmnumber{ #2}\thmnote{ (#3)}}%

\theoremstyle{abcd}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}[theorem]{corollary}













\tcbset{qrboxstyle/.style={
		enhanced jigsaw,	%
		colback=gray!20,
		colframe=gray!40,
		arc=0mm,
		boxrule=1pt,		%
		left=1pt,
		right=1pt,
		topsep at break=1mm,			%
		top=1pt,		%
		bottom=0mm,		%
		breakable,		%
		parbox = false		%
		}}


\newcommand{\resultbox}[1]{
\begin{tcolorbox}[
	enhanced jigsaw,		%
	colback=red!5,
	colframe=red!75!black,	
	arc=0mm,
	left skip=-1mm,
	right skip=-1mm,	
	left=0mm,
	topsep at break=1mm,			%
	right=0mm,
	top=0mm,
	bottom=0mm,		%
	breakable,		%
	parbox = false		%
]
\emph{#1}
\end{tcolorbox}
}


\newcounter{resultboxenv}

\newsavebox{\coloredbgbox}
\newenvironment{resultboxenv}{
	\begin{lrbox}{\coloredbgbox}
		\begin{minipage}{\dimexpr1\linewidth-2\fboxsep-2\fboxrule\relax}
			\refstepcounter{resultboxenv}
			\emph{Result \theresultboxenv.}
			\itshape
		}
  		{
		\end{minipage}
	\end{lrbox}
	\begin{center}
		\fcolorbox{black}{black!05}{\usebox{\coloredbgbox}}
	\end{center}
}



\newtheorem{resultW}{Result}

\renewenvironment{resultW}[1][]
{%
\par\noindent
  {\textbf{Result \arabic{resultW}#1.}
  \stepcounter{resultW}}%
  \begin{itshape}%
}%
{\end{itshape}
}
\setcounter{resultW}{1}

\newtheorem{resultE}{Pilot Result}

\renewenvironment{resultE}[1][]
{%
\par\noindent
  {\textbf{Pilot Result \arabic{resultE}#1.}
  \stepcounter{resultE}}%
  \begin{itshape}%
}%
{\end{itshape}
}
\setcounter{resultE}{1}






\renewcommand\dbltopfraction{1} %
\renewcommand\topfraction{1} 	%
\setcounter{dbltopnumber}{8}	%
\setcounter{topnumber}{8}		%






\usepackage{adjustbox}
\def\eox{\unskip\kern 10pt{\unitlength1pt\linethickness{.4pt}$\diamondsuit${}}}   




	





\makeatletter
\DeclareRobustCommand*\uell{\mathpalette\@uell\relax}
\newcommand*\@uell[2]{
  \setbox0=\hbox{$#1\ell$}
  \setbox1=\hbox{\rotatebox{10}{$#1\ell$}}
  \dimen0=\wd0 \advance\dimen0 by -\wd1 \divide\dimen0 by 2
  \mathord{\lower 0.1ex \hbox{\kern\dimen0\unhbox1\kern\dimen0}}
}
\makeatother




\usepackage{titlesec}
\titleformat{\subsubsection}[runin]
  {\normalfont\normalsize\bfseries}{\thesubsubsection}{1em}{}[.]
\titlespacing*{\subsubsection}{0em}{0.5em}{0.3em}


\newcommand{\smallsection}[1]{\vspace{5mm}\noindent\textbf{#1.}} %
\newcommand{\introparagraph}[1]{\textbf{#1.}} %

\newcommand{\ourmethod}{\textsc{QueryVis} \color{red}{TEST TEST TEST TEST !!!!}\xspace}
\renewcommand{\epsilon}{\varepsilon} %
\newcommand{\set}[1]{\{#1\}}                    %
\newcommand{\setof}[2]{\{{#1}\mid{#2}\}}        %

\newcommand{\define}{\stackrel{\textup{\tiny def}}{=}}

\newcommand{\datarule}{{\,:\!\!-\,}} %
\renewcommand{\vec}[1]{\boldsymbol{\mathbf{#1}}}
\newcommand{\transpose}{\intercal}	%

\newcommand{\N}{\mathbb{N}} %
\newcommand{\R}{{\mathbb{R}}} %
\newcommand{\bigO}{{\mathcal{O}}} %
\renewcommand{\O}{{\mathcal{O}}} %
\renewcommand{\P}{{\mathbb{P}}} %
\newcommand{\PP}[1]{\mathbb{P} [ #1 ]} %
\newcommand{\sql}[1]{\textrm{{#1}}}
\newcommand{\datastyle}[1]{\texttt{#1}}






\usepackage{caption}
    
    

\usepackage{bm}

\newcommand{\qv}{QV\xspace}


\newcommand{\formattedurl}[2]{\href{#1}{\small\texttt{#2}}\xspace}







\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{mymauve}{rgb}{0.58,0,0.82}
\definecolor{myred}{rgb}{1,0,0}
\definecolor{mylightblue}{rgb}{0.953, 0.957, 0.980} 	%
\definecolor{mylightblueborder}{rgb}{0.567, 0.627, 0.757} 	%
\definecolor{mylightyellow}{rgb}{0.988, 0.957, 0.863} 	%



\lstset{ 
  backgroundcolor=\color{mylightyellow},   %
  rulecolor=\color{mylightblueborder},         %
  basicstyle=\footnotesize\ttfamily\linespread{0.75}, %
  breakatwhitespace=false,         %
  breaklines=true,                 %
  captionpos=b,                    %
  commentstyle=\color{mygreen},    %
  deletekeywords={...},            %
  escapeinside={\%*}{*)},          %
  extendedchars=true,              %
  frame=single,	                   %
  keepspaces=true,                 %
  numbers=none,                    %
  numbersep=5pt,                   %
  numberstyle=\tiny\color{mygray}, %
  showspaces=false,                %
  showstringspaces=false,          %
  showtabs=false,                  %
  stepnumber=1,                    %
  stringstyle=\color{mymauve},     %
  tabsize=2,	                   %
  title=\lstname,                  %
  classoffset=0,
  morekeywords={SELECT, DISTINCT, FROM, WHERE, AND, AS, ON,},            %
  keywordstyle=\color{blue},       %
  classoffset=1,%
  morekeywords={SELECT},
  keywordstyle=\color{blue},
  classoffset=2,%
  morekeywords={not, exists, in, any, all, OR, UNION, IN, ANY, ALL, NOT, EXISTS, LEFT, JOIN, IS, NULL},
  keywordstyle=\color{myred},
  classoffset=3,%
  morekeywords={test},
  keywordstyle=\color{mymauve},
  classoffset=4,%
  morekeywords={query, block1, block2, block3, block4, qb1, qb2, qb3, qb4, subquery2},
  keywordstyle=\color{gray},  
  classoffset=0,%
}








\RequirePackage{scalerel}
\RequirePackage{tikz}
\usetikzlibrary{svg.path}

\definecolor{orcidlogocol}{HTML}{A6CE39}
\tikzset{
  orcidlogo/.pic={
    \fill[orcidlogocol] svg{M256,128c0,70.7-57.3,128-128,128C57.3,256,0,198.7,0,128C0,57.3,57.3,0,128,0C198.7,0,256,57.3,256,128z};
    \fill[white] svg{M86.3,186.2H70.9V79.1h15.4v48.4V186.2z}
                 svg{M108.9,79.1h41.6c39.6,0,57,28.3,57,53.6c0,27.5-21.5,53.6-56.8,53.6h-41.8V79.1z M124.3,172.4h24.5c34.9,0,42.9-26.5,42.9-39.7c0-21.5-13.7-39.7-43.7-39.7h-23.7V172.4z}
                 svg{M88.7,56.8c0,5.5-4.5,10.1-10.1,10.1c-5.6,0-10.1-4.6-10.1-10.1c0-5.6,4.5-10.1,10.1-10.1C84.2,46.7,88.7,51.3,88.7,56.8z};
  }
}

\RequirePackage{etoolbox}
\DeclareRobustCommand\orcidicon[1]{\href{https://orcid.org/#1}{\mbox{\scalerel*{
\begin{tikzpicture}[yscale=-1, transform shape]
    \pic{orcidlogo};
\end{tikzpicture}
}{|}}}}
 




\newcommand{\equal}{\!=\!}

\let\oldin\in
\renewcommand{\in}{\!\oldin\!}
\renewcommand{\L}{\mathcal{L}}

\newcommand{\rep}{\textrm{rep}}
\newcommand{\ex}{\textrm{exp}}

\newcommand{\RA}{\textsf{RA}}
\newcommand{\NDRA}{\RA^{*}}
\newcommand{\NDRAPlain}{\RA*}
\newcommand{\NDRAA}{\RA^{*\antijoin}}

\newcommand{\Datalog}{\textsf{Datalog}}
\newcommand{\DatalogN}{\Datalog^{\neg}}
\newcommand{\DatalogND}{\Datalog^{*}}

\newcommand{\FOL}{\textsf{FOL}}
\newcommand{\DRC}{\textsf{DRC}}
\newcommand{\TRC}{\textsf{TRC}}
\newcommand{\ENCTRC}{\textsf{ENC-TRC}}
\newcommand{\ENTRC}{\textsf{EN-TRC}}
\newcommand{\RC}{\textsf{RC}}
\newcommand{\NDTRC}{\TRC^{*}}
\newcommand{\NDTRCPlain}{\TRC*}

\newcommand{\SQL}{\textsf{SQL}\xspace}
\newcommand{\NDSQL}{\textsf{SQL}^{*}}


\newcommand{\NRD}{\textsf{RD}^{*}}
\newcommand{\RD}{\textsf{RD}}

\newcommand{\QBE}{\textsf{QBE}}


\newcommand{\queryviz}{\textsf{QueryVis}}










\newcommand{\diagram}{\textrm{Relational Diagram}}
\newcommand{\diagrams}{\textrm{Relational Diagrams}}
\newcommand{\systemx}{\textsf{RepresentationB}}

\newcommand{\diagramNDnomath}{\texorpdfstring{\textsf{Relational Diagram}$^{*}$}{\textsf{Relational Diagram*}}}

\newcommand{\diagramsNDnomath}{\texorpdfstring{\textsf{Relational Diagrams}$^{*}$}{\textsf{Relational Diagrams*}}}
\newcommand{\diagramsND}{{\textsf{Relational Diagrams}^{*}}}	%














\definecolor{carfigORcolor}{HTML}{e36c1a}	%
\definecolor{carfigBLUEcolor}{HTML}{2b8dcf}	%

\newcommand{\h}[1]{\textcolor{red}{#1}} 	%
\newcommand{\horange}[1]{\textcolor{carfigORcolor}{#1}} 	%
\newcommand{\hblue}[1]{\textcolor{carfigBLUEcolor}{#1}} 	%

\newcommand{\var}{\mathit{var}} 		
\newcommand{\const}{\mathit{const}} 	

\newcommand{\symb}{\bullet\;} 	

\newcommand{\antijoin}{\triangleright}

\newcommand{\tablesandattributes}{\textbf{Tables \& attributes}\xspace}
\newcommand{\constqualifications}{\textbf{Selection predicates}\xspace}
\newcommand{\joinattr}{\textbf{Join predicates}\xspace}
\newcommand{\quantifiers}{\textbf{Quantifiers}\xspace}
\newcommand{\nestingorder}{\textbf{Nesting order}\xspace}

\newcommand{\ittablesandattributes}{\emph{Tables \& attributes}\xspace}
\newcommand{\itconstqualifications}{\emph{Selection predicates}\xspace}
\newcommand{\itjoinattr}{\emph{Join predicates}\xspace}
\newcommand{\itquantifiers}{\emph{Quantifiers}\xspace}
\newcommand{\itnestingorder}{\emph{Nesting order}\xspace}

\newcommand{\true}{\mathsf{true}} 	
\newcommand{\false}{\mathsf{false}} 	

\definecolor{selPredicateColor}{HTML}{FFFFFF} 
\definecolor{selectBoxColor}{HTML}{BFBFBF}
\definecolor{unaryBuiltInPredicate}{HTML}{5A9AD4}		%
\definecolor{unaryBuiltInPredicatesimple}{HTML}{ccdcf1} %
\definecolor{binaryBuiltInPredicate}{HTML}{ED7C30}		%
\definecolor{binaryBuiltInPredicatesimple}{HTML}{ffd3b8}%

\setlength{\fboxsep}{2pt}
\newcommand{\selPredicateBox}[1]{\fcolorbox{black}{selPredicateColor}{\textcolor{black}{#1}}}
\newcommand{\tableBox}[1]{\fcolorbox{black}{black}{\textcolor{white}{#1}}}
\newcommand{\attributeBox}[1]{\fcolorbox{black}{white}{\textcolor{black}{#1}}}
\newcommand{\selectBox}{\fcolorbox{black}{selectBoxColor}{\textcolor{white}{Q}}}


\newcommand{\E}{\mathcal{E}}
\renewcommand{\S}{\mathcal{S}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\schema}{\textsf{schema}}




\newlist{pfparts}{description}{1}
\setlist[pfparts,1]{%
    font=\normalfont\textsf,
    itemindent=2pt,
    wide,
    itemsep=.5em,topsep=.5em,
    labelsep=0.75ex
}
\makeatletter
\def\namedlabel#1#2{\begingroup
    #2%
    \def\@currentlabel{#2}%
    \phantomsection\label{#1}\endgroup
}
\makeatother





\newcommand{\osfpreprintplain}{osf.io/btszh}
\newcommand{\osfsupplementplain}{osf.io/mycr2}
\newcommand{\osfpreregplain}{osf.io/mycr2}

\newcommand{\osfpreprint}{\formattedurl{https://\osfpreprintplain}{\osfpreprintplain}}
\newcommand{\osfpreprintlong}{\formattedurl{https://\osfpreprintplain}{https://\osfpreprintplain}}

\newcommand{\osfsupplement}{\formattedurl{https://\osfsupplementplain}{\osfsupplementplain}}
\newcommand{\osfsupplementlong}{\formattedurl{https://\osfsupplementplain}{https://\osfsupplementplain}}

\newcommand{\osfprereg}{\formattedurl{https://\osfpreregplain}{\osfpreregplain}}


\usepackage{xurl}%


\newcommand{\anchor}[1]{{#1}} 	%

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,fill=black,draw,text=white,inner sep=1.2pt] (char) {#1};}} 			

\newcommand*\builtinlabel[1]{\tikz[baseline=(char.base)]{
	\node[shape=circle,fill=white,draw,text=black,inner sep=0.4pt] (char) {#1};}} 			
	

